Fast binary embeddings, and quantized compressed sensing with structured matrices

This paper deals with two related problems, namely distance-preserving binary embeddings and quantization for compressed sensing . First, we propose fast methods to replace points from a subset $\mathcal{X} \subset \mathbb{R}^n$, associated with the Euclidean metric, with points in the cube $\{\pm 1\}^m$ and we associate the cube with a pseudo-metric that approximates Euclidean distance among points in $\mathcal{X}$. Our methods rely on quantizing fast Johnson-Lindenstrauss embeddings based on bounded orthonormal systems and partial circulant ensembles, both of which admit fast transforms. Our quantization methods utilize noise-shaping, and include Sigma-Delta schemes and distributed noise-shaping schemes. The resulting approximation errors decay polynomially and exponentially fast in $m$, depending on the embedding method. This dramatically outperforms the current decay rates associated with binary embeddings and Hamming distances. Additionally, it is the first such binary embedding result that applies to fast Johnson-Lindenstrauss maps while preserving $\ell_2$ norms. Second, we again consider noise-shaping schemes, albeit this time to quantize compressed sensing measurements arising from bounded orthonormal ensembles and partial circulant matrices. We show that these methods yield a reconstruction error that again decays with the number of measurements (and bits), when using convex optimization for reconstruction. Specifically, for Sigma-Delta schemes, the error decays polynomially in the number of measurements, and it decays exponentially for distributed noise-shaping schemes based on beta encoding. These results are near optimal and the first of their kind dealing with bounded orthonormal systems.

==> binaryembedding.tex <==
\section{Main results on binary embeddings} \label{sec:binary}
We are now ready to present our main results on binary (and more general) embeddings, showing that Algorithm \ref{alg:binary_embedding} yields quasi-isometric embeddings that preserve \emph{Euclidean} distances. We start with the case of finite sets, as our results are stronger in this setting, and we next present an analysis of our methods for infinite sets.  
%Low distortion embeddings have played an important role in the recent applications of signal processing and machine learning as they transform signals in high dimensions signals to low-dimensional ones while preserving geometric properties. The benefits of such embeddings include the potential for reduced storage space and computational time associated with the signals, as a direct consequence of the dimensionality reduction. Perhaps one of the most important embeddings is given by the Johnson-Lindenstrauss (JL) lemma \cite{JL} which shows that one can embed $N$ points in $\R^n$ into a $m=O(\delta^{-2}\log N)$-dimensional space and simultaneously preserve pairwise Euclidean distance up to $\delta$-Lipschitz distortion. %Although the embedded signals are in lower-dimensional space, we still need an enormous disk size to store them. 
%More recently, binary embeddings   have attracted a lot of attention in signal processing and machine learning communities \cite{WTF2009, RL2009, SH2009, LWKC2011, GL2013, YBKGC2015}, in part due to theoretical interest, and in part motivated by the potential benefits of further reductions in memory requirements and computational time. Roughly speaking, they are nonlinear embeddings that map high dimensional signals into a discrete cube in lower-dimensional space. As each signal is now represented by a short binary code, the memory needed for storing the entire data set is reduced considerably.
%
%%Let us now explain the binary embedding problem in more details. 
%To be more precise, let $\mathcal{T}$ be a set of vectors in $\R^n$ and let $\{-1, 1\}^m$ be the binary cube. Given a distance $d_{\T}$ on $\T$, an $\alpha$-binary embedding of $\X$, is a map $f: \T \to \{-1, 1\}^m$ with an associated function $d$ on $\{-1, 1\}^m$ so that 
%\[
%	%|d(f(w),f(\tilde{w} )) - d_{\X}(w, \tilde{w})| \leq \alpha \qquad \text{for all } w, \tilde{w} \in \X,
%	d_{\X}(x, \tilde{x}) - \alpha \leq d(f(x), f(\tilde{x})) \leq d_{\X}(x, \tilde{x}) + \alpha, \qquad \text{for all } x, \tilde{x} \in \T.
%\]
%Recent works have shown that there exist such $\alpha$-binary embeddings \cite{JLBB2013, PV2013, PV2014, YCP2015}. More precisely, with the angular distance $d_{\X}(x, \tilde{x}) = \arccos(\|x\|_2^{-1}\|\tilde{x}\|_2^{-1}\inner{x, \tilde{x}})$, they consider the following map
%\begin{equation}\label{sign function}
%	f_A(x) = \sign(Ax),
%\end{equation}
%where $A$ is an $m\times n$ matrix whose entries are independent standard Gaussian random variables, and $\X$ a finite set of $N$ points in the unit sphere $S^{n-1}$. Then with probability exceeding $1 - \eta$, $f_A$ is a $\alpha$-binary embedding for $\X$ into $\{-1, 1\}^m$ associated with the normalized Hamming distance $d_H(q, \tilde{q}) = \frac{1}{2m}\sum_{i}|q_i - \tilde{q}_i|$, provided that ${m\gtrsim \alpha^{-2}\log(N/\eta).}$ 
%
%
%
%
%\RSnote{this paragraph needs a little love}
%While achieving the optimal bit complexity as shown in \cite{YCP2015}, the above binary embedding is impractical as $A$ is the Gaussian matrix. As known, such matrix is dense and thus makes matrix-vector multiplication slow. As a result, researchers have tried to design other binary embeddings which can be implemented more efficiently. For example, such embeddings include circulant binary embedding \cite{YBKGC2015, OTH2017, DS2016}, structured hashed projections \cite{CCBJKL2016}, binary embeddings using on Walsh-Hadamard matrix and partial Gaussian Toeplitz matrices with random column flips \cite{YCP2015}, etc. To our knowledge, all of these results use the sign function \eqref{sign function} or Memoryless Scalar Quantization to quantize the measurements. While being simple, this quantization method cannot improve when we have more measurements, i.e., when $m$ increases, as discussed in {Section \ref{quantization}}. Moreover, this method does not work when we have two signals with the same direction but different lenghts.
%
%We resolve these above issues by extending the noise-shaping quantization approaches to the binary embedding problem. First, we introduce the \emph{quasi-isometric} embedding.
%
%\begin{definition}[see, e.g., \cite{BGBL2008}]
%A function $f: \mathcal{X} \to\mathcal{Y}$ is called a \emph{quasi-isometry} between metric spaces $(\mathcal{X}, d_{\mathcal{X}})$ and $(\mathcal{Y}, d_{\mathcal{Y}})$ if there exist $C > 0$ and $D \geq 0$ such that
%\[
%	\frac{1}{C}d_{\X}(x, \tilde{x}) - D \leq d_{\mathcal{Y}}(f(x), f(\tilde{x})) \leq Cd_{\X}(x,\tilde{x}) + D
%\]
%for all $x, \tilde{x} \in \X,$ and $E > 0$ such that $d_{\mathcal{Y}}(y, f(x)) < E$ for all $y \in \mathcal{Y}.$
%\end{definition}
%
%\begin{definition}\label{def: pseudometric}
%Let $\widetilde{V} := \frac{1}{\|v\|_2\sqrt{p}}I_p\otimes v$ be a normalized condensation operator. Let $\mathcal{C} = \{-1,1\}^m$ be a discrete cube in $\R^m$. We define a \emph{pseudo-metric} $d_{\widetilde{V}}$ on $\mathcal{C}$ by \[ d_{\widetilde{V}}(q, \tilde{q}) = \|V(q - \tilde{q})\|_2.\] 
%\end{definition}

%\subsection{ Binary embeddings of finite sets}
\begin{theorem}[{\bf Binary embeddings of finite sets}]\label{thm: bin embed finite}
 %such that $\alpha < \tilde{\alpha}/4.$ 
Consider a finite set $\T \subset B_2^n$  and fix an error tolerance $\alpha \in (0, 1)$.  Suppose that for integers $p$ and $m$, $p \leq m$ and $\lambda = m/p$ is an integer and let  $\Phi \in \R^{m\times n}$ be as in Construction \ref{distribution} and $D_\epsilon$ be an $n\times n$ diagonal matrix with i.i.d. random sign entries. Let $\Q: \R^m \to \{\pm 1\}^m$, be a stable quantization scheme that corresponds either to $r$th order $\Sigma\Delta$ quantization or to distributed noise shaping quantization as in Definitions \ref{SDcond} and \ref{Beta_cond} respectively. Let $v\in{\R^\lambda}, \widetilde{V}\in \R^{p\times m}$ be the associated condensation vector, and condensation matrix.

 Define a map $f:\T \to \{\pm 1\}^m$ by $f = \Q\circ\Phi\circ D_\epsilon$. Assume that $k \geq 40(\log(8|\T|) + \mu)$. Then there exist absolute constants $C_1$ and $C_2 > 0$ such that if
\[ m \geq p \geq C_1 \frac{k(\log^4 n + \gamma^2\mu)}{\alpha^2},\]
the map $f$ satisfies
\[ \big|d_{\widetilde{V}}(f(x), f(\tilde{x})) - \|x - \tilde{x}\|_2\big| \leq {\alpha}\|x - \tilde{x}\|_2 + C_2\eta\]
with probability exceeding $1 - 2e^{-\mu}.$ Here, $\gamma := \|v\|_1/\|v\|_2.$ \RSnote{State exactly what $\eta$ is here, in both cases. How does it relate to $\gamma$?}
\end{theorem}

%\begin{theorem}\label{thm: bin embed finite}
%Fix $\alpha > 0$. Let $\T \subseteq B_2^n \subset \R^n$ be a finite set of points. Let $(\Q_{\Sigma\Delta}^{(r)}, v_{\Sigma\Delta}^{(r)}, \widetilde{V}_{\Sigma\Delta}^{(r)})$ and $(\Q_{\beta}, v_{\beta}, \widetilde{V}_{\beta})$ be the quantization-reconstruction schemes defined in Section \ref{sec:Sigma Delta} and Section \ref{sec:distributed}, respectively. Let $\Phi$ be constructed as in Construction \ref{distribution} (with respected to a real unitary matrix). Let $D_\epsilon$ be an $n\times n$ diagonal matrix with i.i.d. random sign entries which is independent of $\Phi$. There exist absolute constants $C_1, C_2 > 0$ and a map $f:\mathcal{T} \to \{-1, 1\}^m$ defined by $f = \Q_{\Sigma \Delta}\circ\Phi\circ D_{\epsilon}$ (or $f = \Q_{\beta}\circ\Phi\circ D_{\epsilon}$) such that for $\eta := \lambda^{-r + 1/2}$ (or $\eta = \beta^{-\lambda}$) we have 
%\[ \left|d_{\widetilde{V}}(f(x), f(\tilde{x})) - d_{\ell_2}(x, \tilde{x}) \right| \leq \max\{\sqrt{\alpha}, \alpha\}d_{\ell_2}(x, \tilde{x}) + C_1\delta\eta, \quad\text{for all } x, \tilde{x} \in \T, \]
%with probability at least $1 - 2e^{-\mu}$ whenever
%%\[ m\geq p \geq C(1 + \gamma^2\mu + \gamma^2)k\log^4 n \frac{\max\left\{1, \frac{\omega^2(\T - \T)}{(\rad(\T - \T))^2}\right\}}{\alpha^2}.\]
%\[ m \geq p \geq C_2\frac{\log(4|\T|)(\log^4 n + \gamma^2 \mu)}{\alpha^2}.\]
%\end{theorem}

\begin{remark}\RSnote{ Comment on how we get better dimensions (and worse probability) if we just use Markov.} \end{remark}
\begin{proof}
The proof is simply an implication of Theorem \ref{thm:KrahmerWard} indicating that RIP matrices with randomized column signs provide Johnson-Lindenstrauss embeddings, and our main technical result, Theorem \ref{main theorem}, showing that our matrices $\widetilde{V}\Phi$ satisfy the appropriate RIP.  Indeed, by Theorem \ref{main theorem}, $\widetilde{V}\Phi$ satisfies $(\alpha, k)$-RIP with probability exceeding $1 - e^{-\mu}.$ Hence by Theorem \ref{main theorem}, with probability at least $1 - 2e^{-\mu}$, the matrix $\widetilde{V}\Phi D_\epsilon$ satisfies
\[ 
	\big|\|\widetilde{V}\Phi D_\epsilon (x - \tilde{x})\|_2^2 - \|x - \tilde{x}\|_2^2\big| \leq \tilde{\alpha}\|x - \tilde{x}\|_2^2
\]
which yields
\[ 
	\big|\|\widetilde{V}\Phi D_\epsilon (x - \tilde{x})\|_2 - \|x - \tilde{x}\|_2\big| \leq \tilde{\alpha}\|x - \tilde{x}\|_2
\]
simultaneously for all $x, \tilde{x} \in\T.$ \RSnote{what is $\widetilde{\alpha}?$}

Note that we can bound the quantization errors by \RSnote{Why? Insert an equation or lemma reference, or a one line argument}
\[
	\|\widetilde{V}f(x) - \widetilde{V}\Phi D_\epsilon\, x\|_2 \leq \eta \quad \text{and}\quad \|\widetilde{V}f(\tilde{x}) - \widetilde{V}\Phi D_\epsilon\, \tilde{x}\|_2 \leq \eta. 
\]
Therefore, by the triangle inequality
\begin{align*}
\big|d_{\widetilde{V}}(f(x), f(\tilde{x})) - \|x - \tilde{x}\|_2\big| &\leq \big|d_{\widetilde{V}}(f(x), f(\tilde{x})) - \widetilde{V}\Phi D_\epsilon\, (x - \tilde{x})\big| + \big|\widetilde{V}\Phi D_\epsilon\, (x - \tilde{x}) - \|x - \tilde{x}\|_2\big|\\
&\leq 2\eta + \tilde{\alpha}\|x - \tilde{x}\|_2.
\end{align*}





\end{proof}


%\THnote{measurement $y$ needs to be bounded to apply noise shaping, so $x$ has to be in some bounded set, says $B_2^n$?}
\begin{theorem}[{\bf Binary embeddings of general sets}]\label{thm: bin embed}
%Fix $\alpha > 0$. Let $\T \subseteq B_2^n \subset \R^n.$ Let $(\Q_{\Sigma\Delta}^{(r)}, v_{\Sigma\Delta}^{(r)}, \widetilde{V}_{\Sigma\Delta}^{(r)})$ and 
%$(\Q_{\beta}, v_{\beta}, \widetilde{V}_{\beta})$ be the quantization-reconstruction schemes defined in Section \ref{sec:Sigma Delta} and Section \ref{sec:distributed}, respectively. Let $\Phi$ be constructed as in Construction \ref{distribution} (with respected to a real unitary matrix). Let $D_\epsilon$ be an $n\times n$ diagonal matrix with i.i.d. random sign entries which is independent of $\Phi$. 
Consider the same setup as Theorem \ref{thm: bin embed finite} albeit now with \emph{any} set $\T \subset B_2^n$.  
Suppose that \[ m\geq p \geq C(1 + \gamma^2\mu + \gamma^2)k\log^4 n \frac{\max\left\{1, \frac{\omega^2(\T - \T)}{(\rad(\T - \T))^2}\right\}}{\alpha^2}.\]
%
%Suppose that for integers $p$ and $m$, $p \leq m$ and $\lambda = m/p$ is an integer and let  $\Phi \in \R^{m\times n}$ be as in Construction \ref{distribution} and $D_\epsilon$ be an $n\times n$ diagonal matrix with i.i.d. random sign entries. Let $\mathcal{A}$ be a quantization alphabet used in the stable quantization scheme $\Q: \R^m \to \mathcal{A}^m$, where $\mathcal{Q}$ corresponds either to $r$th rder $\Sigma\Delta$ quantization or to distributed noise shaping quantization as in Definitions \ref{SDcond} and \ref{Beta_cond} respectively. Let $v\in{\R^\lambda}, \widetilde{V}\in \R^{p\times m}$ be the associated condensation vector, and condensation matrix.
%
%
Then, with probability at least $1 - 2e^{-\mu}$, the map $f:\mathcal{T} \to \{-1, 1\}^m$ given by $f = \Q \circ\Phi\circ D_{\epsilon}$  ensures that
\[ \left|d_{\widetilde{V}}(f(x), f(\tilde{x})) - d_{\ell_2}(x, \tilde{x}) \right| \leq \max\{\sqrt{\alpha}, \alpha\}\rad(\T - \T) + C\delta\eta, \quad\text{for all } x, \tilde{x} \in \T. \]


\end{theorem}
%Hereby, ; and $\omega(\T)$ denotes the Gaussian mean width of a set $\T$ defined as follows.


\subsection*{Proof of Theorem \ref{thm: bin embed}}



%\THnote{Gaussian width complex setting?????}
%\begin{definition}
%For a set $\mathcal{T} \subset \R^n$, the \emph{mean width} $\omega(\mathcal{T})$ is defined by
%\[
%	\omega(\mathcal{T}) := \EE[\sup_{v\in\mathcal{T}} \langle v, g\rangle]
%\]
%where $g$ is a standard Gaussian random vector in $\R^n.$
%\end{definition}

\begin{theorem}
Consider $\widetilde{V}\Phi = V\Lambda A \in \R^{p\times n}$ where $\Lambda$ is a $m\times m$ random sign diagonal matrix and $A$ is drawn from a real BOS or PCE. Then $\widetilde{V}\Phi$ satisfies Multiresolution RIP with sparsity $k$ and distortion $\tilde{\alpha} > 0$ with probability $1 - e^{-\mu}$ whenever
\[
	m \geq p \geq C(1 + \gamma^2 \mu + \gamma^2)\frac{k\log^4 n}{\widetilde{\alpha}^2}.
\]
\end{theorem}
\begin{proof}
Use Theorem \eqref{main theorem} and union bound with $L = \lceil \log_2 n \rceil$. Additionally, use change of variable for $\mu \mapsto \mu + \log L.$
\end{proof}


\begin{theorem}[Oymak-Recht-Soltanolkotabi]
Let $\mathcal{T} \subset \R^n$ and suppose the matrix $H\in\R^{m\times n}$ obeys the Multiresolution RIP with sparsity and distortion levels 
\[
	s = 150(1 + \eta) \quad\text{and}\quad \tilde{\alpha} = \frac{\alpha\cdot\rad(\T)}{C\max\{\rad(\mathcal{T}, \omega(\mathcal{T})\}},
\]
with $C > 0$ an absolute constant. Then, for a diagonal matrix $D$ with an i.i.d. random sign pattern on the diagonal, the matrix $A = HD$ obeys
\[ \sup_{x\in\mathcal{T}}\left|\|Ax\|_2^2 - \|x\|_2^2\right| \leq \max\{\alpha, \alpha^2\}(\rad(\mathcal{T}))^2,\]
with probability at least $1 - e^{-\eta}$.
\end{theorem}

\begin{theorem} 
Let $\T \subseteq B_2^n \subset \R^n.$ Consider $\widetilde{V}$ and $\Phi = \Lambda A \in\R^{m\times n}$, where $A$ is drawn from a real BOS or PCE. Let $D_\epsilon$ be an $n\times n$ diagonal matrix with i.i.d. random sign entries which is independent of $\Lambda$ and $A$. Then 
\[
	\sup_{x\in\T}\left|\|\widetilde{V}\Phi D_ {\epsilon} x\|_2^2 - \|x\|_2^2 \right| \leq \max\{\alpha, \alpha^2\}(\rad(\T))^2,
\]
with probability at least $1 - 2e^{-\mu}$ whenever
\[ m \geq C(1 + \gamma^2\mu + \gamma^2)k\log^4 n \frac{\max\left\{1, \frac{\omega^2(\T)}{(\rad(\T))^2}\right\}}{\alpha^2}.\]
\end{theorem}

Now we are ready to prove Theorem \ref{thm: bin embed}. First, we need the following elementary inequality.
\begin{lemma}
\[ \max\{|z - 1|, |z - 1|^2\} \leq |z^2 - 1| \leq 3\max\{|z - 1|, |z - 1|^2\}, \quad \forall z \geq 0.\]
\end{lemma}
Then for all $x\in \T$
\begin{equation}
\left| \frac{\|\widetilde{V}\Phi D_{\epsilon} x\|_2}{\|x\|_2} - 1 \right|^2 \leq \left| \frac{\|\widetilde{V}\Phi D_{\epsilon} x\|_2^2}{\|x\|_2^2} - 1 \right| \leq \frac{\max\{\alpha, \alpha^2\}(\rad(\T))^2}{\|x\|_2^2}.
\end{equation}
This yields
\begin{equation}
\left|\|\widetilde{V}\Phi D_{\epsilon} x\|_2 - \|x\|_2 \right| \leq \max\{\sqrt{\alpha}, \alpha\}\rad(\T) \quad x\in\T.
\end{equation}
Define an embedding $f:\R^n \to \mathcal{C}^p$ by \[ f = \widetilde{V}\circ\Q\circ\Phi\circ D_{\epsilon},\]
where $\mathcal{C}^p = V\A^m.$ Then for any $w$ and $v$ in $\T$ we have
\begin{align*}
\left|\|f(w) - f(v)\|_2 - \|w - v\|_2 \right| &= \left|\|\widetilde{V}\Q(\Phi D_{\epsilon} w) - \widetilde{V}\Q(\Phi D_{\epsilon} v)\|_2 - \|w - v\|_2  \right|\\
&= \left|\|(\widetilde{V}\Phi D_{\epsilon} w - \widetilde{V}\Phi D_{\epsilon} v) - (\widetilde{V}Hu_w - \widetilde{V}Hu_v)\|_2 - \|w - v\|_2\right|\\
&\leq \left| \|\widetilde{V}\Phi D_{\epsilon} (w - v)\|_2 - \|w - v\|_2\right| + \left|\widetilde{V}H(u_w - u_v)\right|\\
&\leq \max\{\sqrt{\alpha}, \alpha\}\rad(\T - \T) + C\eta\delta.
\end{align*}
Here $\eta = \lambda^{-r + 1/2}$ if we use the $\Sigma\Delta$ quantization scheme; and $\eta = \beta^{-\lambda}$ if we use the distributed noise-shaping scheme.

